A Distributionally Robust Multi-agent Reinforcement Learning Framework for Intelligent Intersection Control

Multi-agent reinforcement learning (MARL) has emerged as a promising approach for traffic signal control. However, standard MARL policies typically optimize for expected returns under nominal conditions, leaving them highly vulnerable to spatial-temporal demand shifts and catastrophic congestion under adverse scenarios. To address this critical limitation, this paper proposes an algorithm-agnostic Distributionally Robust (DR) MARL framework integrating an adaptive Contextual-Bandit Worst-Case Estimator (CB-WCE). Operating on a slower timescale, the CB-WCE co-evolves with the traffic controllers by dynamically generating adversarial demand mixtures during training. This steers the learning process to fortify policies against bottleneck scenarios without requiring modifications to the underlying MARL architectures. The framework is evaluated across value-based, actor-critic, and policy-gradient methods on both a synthetic 5x5 grid and a heterogeneous Monaco City network. Empirical results demonstrate that the DR framework prevents unbounded queue growth and profoundly enhances both worst-case robustness and average-case efficiency. Notably, for the Proximal Policy Optimization (PPO) architecture in the Monaco environment, on average, robust retraining reduced the worst-case queue length by 74.39% and improved the average-case network-wide queue length by 75.45%. Furthermore, the retrained policies exhibit strong zero-shot generalization to unseen traffic distributions, highlighting the framework's scalability and potential for resilient real-world urban deployment.

==> backup.tex <==
% -------------------------------------------------------------------------------------------

% Backup related work:

\section{Related Work}
\label{sec:related_work}
In this section, we review prior work on reinforcement-learning (RL) based traffic signal control and motivate our contribution within this literature. For traffic signal control problems, RL methods are typically distinguished by (i) how the control task is formulated (single-intersection versus network-level), (ii) the learning paradigm (value-based, policy-gradient, or actor--critic), and (iii) the coordination mechanism used to address scalability and partial observability in multi-intersection settings. We focus in particular on multi-agent reinforcement learning (MARL) approaches for large-scale networks, since our study builds directly on established MARL baselines and investigates how their performance can be improved under traffic-demand variability and distribution shift.

\subsection{DRL and MARL for Traffic Signal Control}
\label{subsec:drl_marl_tsc}

Reinforcement learning has been widely studied for traffic signal control, with formulations ranging from isolated intersections to large-scale networks. We briefly review representative deep RL and multi-agent RL approaches, emphasizing how modeling choices for state, action, and coordination have evolved toward scalable network control.

\subsubsection{Deep RL at Isolated Intersections}
A simple and widely studied formulation of RL-based traffic signal control considers isolated intersections, where deep function approximation enables richer state representations than traditional detector-based features. \cite{genders2016} introduced a DQN controller in \textsc{SUMO} using an image-like discretization of approaching traffic processed by a CNN, while \cite{mousavi2017} investigated both value-based and policy-gradient methods operating directly on visual snapshots. Moving toward more structured yet scalable representations, \cite{wei2018intellilight} proposed IntelliLight, which encodes lane occupancy, waiting time, and phase context into an image-like state and uses a DQN to decide whether to \emph{hold} or \emph{switch} to the next legal phase. Across these studies, the control loop follows a common pattern: compact lane- or image-based \emph{states}, discrete \emph{actions} over phases or switching decisions, and \emph{rewards} shaped to reduce delay, queues, or stops. While these results demonstrate the effectiveness of deep RL for single-junction control, they do not address coordination and non-stationarity in traffic networks, motivating multi-agent formulations for large-scale signal control.

\subsubsection{Multi-Agent Formulations for Network Control}
To scale RL-based traffic signal control beyond isolated intersections, a substantial body of work has adopted multi-agent reinforcement learning (MARL), where each intersection is controlled by an autonomous agent that observes local traffic conditions and selects signal actions while interacting with neighboring agents through the shared environment. Early studies such as \cite{van2016coordinated} demonstrated that decentralized agents can achieve coordinated behavior across arterial networks using limited local information, highlighting MARL as a viable alternative to centralized optimization for large-scale systems.

\subsubsection{Deep MARL and Learned Coordination}
With the maturation of deep RL, MARL approaches increasingly leverage function approximation and structured state representations. \cite{wei2019presslight} proposed PressLight, a decentralized DQN-based controller that incorporates pressure-based traffic features to improve stability and scalability, while \cite{wei2019colight} extended this idea using graph attention to explicitly model spatial dependencies among neighboring intersections. Similarly, \cite{chu2019multi} introduced a scalable multi-agent deep RL framework in which intersections learn from local queue, waiting-time, and phase-timer observations, achieving consistent improvements over fixed-time and actuated baselines on large grids. More recent work further emphasizes learned coordination mechanisms: \cite{zhang2023learning} formulates traffic signal control as a graph-based MARL problem, using learned message passing to aggregate neighboring states while maintaining decentralized execution.

\subsubsection{Limitations and Open Challenges}
Overall, these MARL methods demonstrate that combining decentralized control with limited information sharing or learned spatial representations can substantially improve network-level performance. However, they also reveal persistent challenges related to non-stationarity, sample efficiency, sensitivity to traffic-demand variability, and robustness under distribution shift—issues that motivate our focus on improving MARL performance under uncertain and heterogeneous traffic conditions.





\subsection{Robust Training for RL-Based Traffic Signal Controllers}
\label{subsec:robust_training}

Traffic-signal controllers trained under a fixed or narrow distribution of traffic conditions often exhibit degraded performance when deployed under distribution shift, such as peak-demand surges, incidents, altered turning ratios, or network disruptions. These shifts change the effective state--transition dynamics and context distribution faced by the controller, causing policies optimized for average-case performance to underperform in rare but consequential regimes. This motivates robustness-aware training objectives that emphasize adverse traffic conditions rather than only typical operating points.

\subsubsection{Robust RL Perspectives}
Robustness in reinforcement learning is commonly formalized through two complementary lenses. In \emph{robust Markov decision processes}, uncertainty sets are defined over transitions and/or rewards, and policies are optimized for worst-case return via min--max dynamic programming \cite{iyengar2005robust,nilim2005robust}. In contrast, \emph{risk-sensitive} approaches optimize tail-aware criteria such as CVaR, emphasizing poor outcomes without requiring an explicit uncertainty set \cite{tamar2015cvar}. In deep RL, these objectives are often approximated through training-time surrogates, including domain randomization, adversarial perturbations \cite{pinto2017rarl}, or hard-trajectory selection methods such as EPOpt, which update on the worst-performing rollouts to approximate a CVaR-like objective \cite{rajeswaran2017epopt}. These approaches share a common principle: reweight learning toward difficult regimes while keeping the underlying optimizer unchanged.

\subsubsection{Context Selection as a Contextual-Bandit Problem}
In traffic signal control, robustness can be pursued by explicitly controlling which traffic regimes are emphasized during training. We view this as a contextual bandit problem, where each \emph{context} (e.g., a demand pattern, turning-ratio profile, or topology configuration) induces a stochastic return under the current policy, and training must adaptively allocate samples across contexts to improve a robustness criterion. Foundational work on contextual bandits formalizes exploration--exploitation and off-policy evaluation under function approximation \cite{langford2008epochgreedy,dudik2011doubly,agarwal2014taming}. In our setting, the selector’s utility corresponds to \emph{negative} policy performance, so the objective is to identify and upweight contexts where the controller performs worst. This perspective aligns with adversarial or group-aware sampling and provides a principled basis for our worst-case estimator, which adaptively concentrates data collection on adverse traffic regimes while remaining lightweight enough to integrate with standard multi-agent RL training pipelines.


\subsubsection{Distributional Robustness and Group Reweighting}
Closely related ideas arise in distributionally robust optimization (DRO), particularly \emph{group DRO}, which improves worst-group performance by upweighting underperforming subpopulations \cite{sagawa2020gdro,hashimoto2018fairness}. In reinforcement learning, this corresponds to treating training as a mixture over contexts and optimizing for the worst-performing group. Recent work extends this formulation to multi-agent settings, showing that reweighting adverse contexts during training can significantly improve worst-case returns without materially degrading average performance \cite{liu2025distributionallyrobustmultiagentreinforcement}. Our approach adopts this philosophy by treating heterogeneous traffic-demand regimes as groups and using a worst-case estimator to guide context selection and weighting during training.

\subsubsection{Robustness in Traffic Signal Control}
Despite strong empirical performance, most RL-based traffic signal control studies evaluate controllers under fixed or mildly perturbed demand patterns, with training and testing conducted on similar traffic distributions \cite{wei2018intellilight,van2016coordinated,wei2019presslight,wei2019colight,chu2019multi}. Only a limited number of works explicitly examine robustness under deliberate distribution shift, such as demand surges, incidents, or altered network conditions, and these studies consistently report substantial performance degradation when policies are deployed outside their training regime. While recent work has begun to explore robustness and generalization in traffic signal control \cite{zhang2023learning,rodrigues2019towards}, systematic mechanisms that explicitly target worst-case performance during training remain relatively underexplored, particularly in large-scale multi-agent settings.


\subsubsection{Positioning of our Approach}
To address these challenges, we pursue robustness through \emph{data-side} reweighting rather than aggressive adversarial optimization. Our method uses a contextual bandit worst-case estimator to adaptively emphasize difficult traffic regimes during training, while leaving the underlying multi-agent RL algorithm unchanged. This design directly targets worst-case performance under demand variability and distribution shift, while maintaining the safety and stability constraints inherent to traffic signal control. In effect, our approach implements a group-distributionally robust training objective that can be applied across value-based and actor--critic multi-agent controllers in large traffic networks.



\subsection{Motivation}
\label{subsec:motivation}

While recent MARL approaches have demonstrated strong average-case performance for large-scale traffic signal control, their robustness under demand variability and distribution shift remains limited. In the broader MARL literature, \cite{liu2025distributionallyrobustmultiagentreinforcement} show that distributionally robust objectives based on reweighting underperforming contexts can substantially improve worst-case performance without resorting to adversarial dynamics. However, directly applying such methods to traffic signal control is challenging due to safety constraints, long temporal dependencies, and the structured heterogeneity of traffic demand. Motivated by this perspective, we treat traffic demand patterns as contexts and introduce a lightweight contextual bandit worst-case estimator that emphasizes difficult regimes during training while remaining compatible with standard multi-agent traffic signal controllers, enabling robust training without modifying the underlying learning algorithms.






% Slightly shorter:

\section{Related Work}
\label{sec:related_work}

In this section, we review prior work on reinforcement-learning (RL) based traffic signal control and position our contribution within this literature. RL approaches for traffic signal control are commonly distinguished by (i) the control scope (isolated intersections versus networks), (ii) the learning paradigm (value-based, policy-gradient, or actor--critic), and (iii) the coordination mechanism used to address scalability and partial observability in multi-intersection settings. Our work builds on multi-agent reinforcement learning (MARL) approaches for large-scale networks and investigates how their performance can be improved under traffic-demand variability and distribution shift.

\subsection{DRL and MARL for Traffic Signal Control}
\label{subsec:drl_marl_tsc}

Reinforcement learning has been widely studied for traffic signal control, with formulations ranging from isolated intersections to large-scale networks.

\subsubsection{Deep RL at Isolated Intersections}

Early work applied deep reinforcement learning to isolated intersections, where deep function approximation enables richer state representations than traditional detector-based features. \cite{genders2016} introduced a DQN controller in \textsc{SUMO} using a CNN-based representation of approaching traffic, while \cite{mousavi2017} explored both value-based and policy-gradient methods operating on visual snapshots. Moving toward structured yet scalable representations, \cite{wei2018intellilight} proposed IntelliLight, which encodes lane occupancy, waiting time, and phase context into an image-like state and applies DQN to decide whether to hold or switch phases. While these studies demonstrate the effectiveness of deep RL for single intersections, they do not address coordination and non-stationarity in traffic networks.

\subsubsection{Multi-Agent Formulations for Network Control}

To scale RL-based signal control to networks, many studies adopt multi-agent reinforcement learning (MARL), where each intersection is controlled by an autonomous agent interacting with neighboring intersections through the shared traffic environment. Early work such as \cite{van2016coordinated} showed that decentralized agents using local observations can achieve coordinated behavior across arterial networks, demonstrating MARL as a viable alternative to centralized optimization for large-scale signal control.

\subsubsection{Deep MARL and Learned Coordination}

With the rise of deep RL, MARL approaches increasingly incorporate function approximation and structured spatial representations. \cite{wei2019presslight} proposed PressLight, a decentralized DQN-based controller using pressure-based traffic features to improve stability and scalability. \cite{wei2019colight} extended this idea with graph attention to model spatial dependencies among neighboring intersections. Similarly, \cite{chu2019multi} introduced a scalable deep MARL framework using local queue, waiting-time, and phase-timer observations, achieving consistent improvements over fixed-time and actuated baselines on large grid networks. More recent work further explores learned coordination mechanisms; for example, \cite{zhang2023learning} formulates traffic signal control as a graph-based MARL problem with message passing between neighboring intersections.

\subsubsection{Limitations and Open Challenges}

Despite strong empirical results, these MARL approaches remain sensitive to traffic-demand variability and distribution shift. Controllers trained under a narrow set of demand conditions may degrade significantly when exposed to atypical traffic regimes, highlighting the need for training approaches that explicitly account for heterogeneous and uncertain traffic demand.

\subsection{Robust Training for RL-Based Traffic Signal Controllers}
\label{subsec:robust_training}

Traffic signal controllers trained under a fixed or narrow demand distribution often perform poorly when deployed under distribution shift, such as peak-demand surges, incidents, or altered turning ratios. These shifts change the effective state--transition dynamics and context distribution faced by the controller, motivating robustness-aware training objectives that emphasize adverse traffic conditions.

\subsubsection{Robust RL Perspectives}

Robustness in reinforcement learning is commonly studied through robust MDP formulations and risk-sensitive objectives. Robust MDPs optimize policies under worst-case transition or reward uncertainty \cite{iyengar2005robust,nilim2005robust}, while risk-sensitive methods optimize tail-aware criteria such as CVaR \cite{tamar2015cvar}. In deep RL, robustness is often approximated through training-time mechanisms such as domain randomization, adversarial perturbations \cite{pinto2017rarl}, or worst-trajectory sampling methods like EPOpt \cite{rajeswaran2017epopt}, which bias learning toward difficult regimes.

\subsubsection{Context Selection as a Contextual-Bandit Problem}

Robustness can also be pursued by controlling which traffic regimes are emphasized during training. We interpret this as a contextual bandit problem, where each context (e.g., a demand pattern or network configuration) induces a stochastic return under the current policy, and training adaptively allocates samples across contexts. Foundational work on contextual bandits studies exploration--exploitation trade-offs and off-policy evaluation under function approximation \cite{langford2008epochgreedy,dudik2011doubly,agarwal2014taming}. In our setting, contexts correspond to traffic-demand regimes, and the selector aims to identify and emphasize scenarios where the controller performs poorly.

\subsubsection{Distributional Robustness and Group Reweighting}

Related ideas arise in distributionally robust optimization (DRO), particularly group DRO, which improves worst-group performance by upweighting underperforming subpopulations \cite{sagawa2020gdro,hashimoto2018fairness}. In reinforcement learning, this corresponds to treating training as a mixture over contexts and optimizing for the worst-performing group. Recent work shows that reweighting adverse contexts during training can significantly improve worst-case returns without substantially degrading average performance \cite{liu2025distributionallyrobustmultiagentreinforcement}. Our approach adopts this philosophy by treating heterogeneous traffic-demand regimes as groups and adaptively reweighting them during training.

\subsubsection{Robustness in Traffic Signal Control}

Despite the success of RL-based traffic signal control, most studies evaluate controllers under fixed or mildly perturbed demand patterns \cite{wei2018intellilight,van2016coordinated,wei2019presslight,wei2019colight,chu2019multi}. Only a limited number of works explicitly examine robustness under deliberate distribution shift \cite{zhang2023learning,rodrigues2019towards}, and these studies consistently report substantial performance degradation when policies are deployed outside their training regime.

\subsection{Motivation}
\label{subsec:motivation}

While recent MARL approaches achieve strong average-case performance for network-level traffic signal control, their robustness under demand variability remains limited. In the MARL literature, \cite{liu2025distributionallyrobustmultiagentreinforcement} show that distributionally robust objectives based on reweighting underperforming contexts can improve worst-case performance without adversarial dynamics. However, applying such methods to traffic signal control is challenging due to safety constraints, long temporal dependencies, and structured demand heterogeneity. Motivated by this perspective, we treat traffic demand patterns as contexts and introduce a lightweight contextual-bandit worst-case estimator that emphasizes difficult regimes during training while remaining compatible with standard multi-agent traffic signal controllers.




















% -------------------------------------------------------------------------------------------


% Backup tables:



\begin{table}[t!]
    \centering
    \caption{Comparison of the baseline IA2C and DR-MARL IA2C performance per group (horizon-and-rollout-averaged).}
    \label{tab:comp}
    \begin{tabular}{|c|cc|cc|}
        \hline
        & \multicolumn{2}{c|}{queue length} & \multicolumn{2}{c|}{average speed} \\
        \cline{2-5}
        groups\rule{0pt}{2.6ex}
        & MARL & DR-MARL & MARL & DR-MARL \\
        \hline
        0 & 80.65 & 83.56 & 3.61 & 3.72 \\
        1 & 83.57 & 94.80 & 3.36 & 3.32 \\
        2 & 217.72 & 177.59 & 2.09 & 2.61 \\
        3 & 164.37 & 173.09 & 2.83 & 2.79 \\
        4 & 138.56 & 135.09 & 2.59 & 2.68 \\
        5 & 137.57 & 143.41 & 2.76 & 2.70 \\
        6 & 175.90 & 151.58 & 2.30 & 2.55 \\
        7 & 157.70 & 142.26 & 2.52 & 2.67 \\  
        8 & 57.51 & 49.08 & 5.41 & 5.83 \\
        9 & 54.23 & 47.72 & 5.56 & 5.92 \\
        10 & 53.05 & 48.90 & 5.68 & 5.88 \\
        \hline
    \end{tabular}
\end{table}

\begin{table}[t!]
    \centering
    \caption{Comparison of the baseline MA2C and DR-MARL MA2C performance per group (horizon-and-rollout-averaged).}
    \label{tab:comp}
    \begin{tabular}{|c|cc|cc|}
        \hline
        & \multicolumn{2}{c|}{queue length} & \multicolumn{2}{c|}{average speed} \\
        \cline{2-5}
        groups\rule{0pt}{2.6ex}
        & MARL & DR-MARL & MARL & DR-MARL \\
        \hline
        0 & 70.33 & 74.03 & 3.83 & 4.07 \\
        1 & 78.02 & 79.16 & 3.62 & 3.92 \\
        2 & 195.72 & 151.13 & 2.41 & 3.03 \\
        3 & 184.80 & 116.92 & 2.74 & 3.51 \\
        4 & 141.58 & 128.96 & 2.51 & 2.78 \\
        5 & 147.68 & 130.49 & 2.47 & 2.74 \\
        6 & 177.50 & 147.41 & 2.14 & 2.64 \\
        7 & 152.38 & 136.41 & 2.48 & 2.85 \\  
        8 & 52.60 & 41.24 & 5.65 & 6.24 \\
        9 & 52.46 & 40.83 & 5.65 & 6.30 \\
        10 & 52.25 & 41.56 & 5.73 & 6.29 \\
        \hline
    \end{tabular}
\end{table}


\begin{table}[t!]
    \centering
    \caption{Relative change in queue length and average speed (in~\%).}
    \label{tab:comp_diff}
    \begin{tabular}{|c|cc|cc|}
        \hline
        & \multicolumn{2}{c|}{IA2C} & \multicolumn{2}{c|}{MA2C} \\
        \cline{2-5}
        groups\rule{0pt}{2.6ex} & queue length & average speed & queue length & average speed \\
        \hline
        0  & 3.61  & 3.11  & 5.27 & 6.25 \\
        1  & 13.45 & -1.21 & 1.46 & 8.06 \\
        2  & -18.43 & 24.67 & -22.78 & 25.68 \\
        3  & 5.30  & -1.64 & -36.72 & 28.30 \\
        4  & -2.53 & 3.83  & -8,91 & 10.77 \\
        5  & 4.25  & -2.19 & -11.64 & 11.07 \\
        6  & -13.78 & 10.68 & -16.95 & 23.28 \\
        7  & -9.79 & 5.83  & -10.48 & 15.12 \\
        8  & -14.66 & 7.73 & -21.60 & 10.49 \\
        9  & -12.01 & 6.47 & -22.18 & 11.47 \\
        10 & -7.83 & 3.66 & -20.46 & 9.64 \\
        \hline
    \end{tabular}
\end{table}





% ----------------------------------------

% Old results tables


\begin{table*}[t!]
\centering
\scriptsize
\caption{Horizon- and rollout-averaged performance of baseline and distributionally robust controllers across demand groups. Absolute values are reported for queue length and average speed; $\Delta$ denotes the relative change of DR-MARL with respect to MARL (in \%).}
\label{tab:bench_combined_ia2c_ma2c}

\begin{tabular}{c ccc ccc ccc ccc}
\toprule
& \multicolumn{6}{c}{IA2C} & \multicolumn{6}{c}{MA2C} \\

\cmidrule(lr){2-7} \cmidrule(lr){8-13}

& \multicolumn{3}{c}{queue length (veh)} 
& \multicolumn{3}{c}{average speed (m/s)}
& \multicolumn{3}{c}{queue length (veh)} 
& \multicolumn{3}{c}{average speed (m/s)} \\

\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}

groups
& MARL & DR-MARL & $\Delta$ (\%)
& MARL & DR-MARL & $\Delta$ (\%)
& MARL & DR-MARL & $\Delta$ (\%)
& MARL & DR-MARL & $\Delta$ (\%) \\

\midrule

0  & 80.65 & 83.56 & 3.61  & 3.61 & 3.72 & 3.11
   & 70.33 & 74.03 & 5.27  & 3.83 & 4.07 & 6.25 \\

1  & 83.57 & 94.80 & 13.45 & 3.36 & 3.32 & -1.21
   & 78.02 & 79.16 & 1.46  & 3.62 & 3.92 & 8.06 \\

2  & 217.72 & 177.59 & -18.43 & 2.09 & 2.61 & 24.67
   & 195.72 & 151.13 & -22.78 & 2.41 & 3.03 & 25.68 \\

3  & 164.37 & 173.09 & 5.30  & 2.83 & 2.79 & -1.64
   & 184.80 & 116.92 & -36.72 & 2.74 & 3.51 & 28.30 \\

4  & 138.56 & 135.09 & -2.53 & 2.59 & 2.68 & 3.83
   & 141.58 & 128.96 & -8.91 & 2.51 & 2.78 & 10.77 \\

5  & 137.57 & 143.41 & 4.25  & 2.76 & 2.70 & -2.19
   & 147.68 & 130.49 & -11.64 & 2.47 & 2.74 & 11.07 \\

6  & 175.90 & 151.58 & -13.78 & 2.30 & 2.55 & 10.68
   & 177.50 & 147.41 & -16.95 & 2.14 & 2.64 & 23.28 \\

7  & 157.70 & 142.26 & -9.79 & 2.52 & 2.67 & 5.83
   & 152.38 & 136.41 & -10.48 & 2.48 & 2.85 & 15.12 \\

8  & 57.51 & 49.08 & -14.66 & 5.41 & 5.83 & 7.73
   & 52.60 & 41.24 & -21.60 & 5.65 & 6.24 & 10.49 \\

9  & 54.23 & 47.72 & -12.01 & 5.56 & 5.92 & 6.47
   & 52.46 & 40.83 & -22.18 & 5.65 & 6.30 & 11.47 \\

10 & 53.05 & 48.90 & -7.83 & 5.68 & 5.88 & 3.66
   & 52.25 & 41.56 & -20.46 & 5.73 & 6.29 & 9.64 \\

\midrule

\textbf{avg}
& \textbf{120.08} & \textbf{113.37} & \textbf{-4.77}
& \textbf{3.52} & \textbf{3.70} & \textbf{5.54}
& \textbf{118.66} & \textbf{98.92} & \textbf{-15.00}
& \textbf{3.57} & \textbf{4.03} & \textbf{14.56} \\

\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[t!]
\centering
\scriptsize
\caption{Horizon- and rollout-averaged performance of baseline and distributionally robust controllers across demand groups. Absolute values are reported for queue length and average speed; $\Delta$ denotes the relative change of DR-MARL with respect to MARL (in \%).}
\label{tab:bench_combined_iqll_ppo}

\begin{tabular}{c ccc ccc ccc ccc}
\toprule
& \multicolumn{6}{c}{IQL-LR} & \multicolumn{6}{c}{PPO} \\

\cmidrule(lr){2-7} \cmidrule(lr){8-13}

& \multicolumn{3}{c}{queue length (veh)} 
& \multicolumn{3}{c}{average speed (m/s)}
& \multicolumn{3}{c}{queue length (veh)} 
& \multicolumn{3}{c}{average speed (m/s)} \\

\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}

groups
& MARL & DR-MARL & $\Delta$ (\%)
& MARL & DR-MARL & $\Delta$ (\%)
& MARL & DR-MARL & $\Delta$ (\%)
& MARL & DR-MARL & $\Delta$ (\%) \\

\midrule

0  & 148.23 & 174.142 & 17.48 & 2.74 & 2.74 & 0
   & -- & -- & -- & -- & -- & -- \\

1  & 164.90 & 201.94 & 22.46 & 2.65 & 2.50 & -5.58
   & -- & -- & -- & -- & -- & -- \\

2  & 351.00 & 75.813 & -78.40 & 1.70 & 7.61 & 347.65
   & -- & -- & -- & -- & -- & -- \\

3  & 172.00 & 44.76 & -73.80 & 3.48 & 7.40 & 112.64
   & -- & -- & -- & -- & -- & -- \\

4  & 286.00 & 14.05 & -95.09 & 1.65 & 3.52 & 113.33
   & -- & -- & -- & -- & -- & -- \\

5  & 242.042 & 111.683 & -53.86 & 2.48 & 3.91 & 57.66
   & -- & -- & -- & -- & -- & -- \\

6  & 119.00 & 135.64 & 13.98 & 2.63 & 3.19 & 21.29
   & -- & -- & -- & -- & -- & -- \\

7  & 252.72 & 144.00 & -43.02 & 1.59 & 3.38 & 112.58
   & -- & -- & -- & -- & -- & -- \\

8  & 60.157 & 49.36 & -17.95 & 6.03 & 8.01 & 32.84
   & -- & -- & -- & -- & -- & -- \\

9  & 47.62 & 95.46 & 100.46 & 6.22 & 6.25 & 0.48
   & -- & -- & -- & -- & -- & -- \\

10 & 51.27 & 21.13 & -58.79 & 6.35 & 9.01 & 41.89
   & -- & -- & -- & -- & -- & -- \\

\midrule

\textbf{avg}
& \textbf{172.27} & \textbf{97.09} & \textbf{-24.23}
& \textbf{3.41} & \textbf{5.23} & \textbf{75.89}
& -- & -- & --
& -- & -- & -- \\

\bottomrule
\end{tabular}
\end{table*}
